Vocal Tract Length Perturbation for Text-Dependent Speaker Verification with Autoregressive Prediction Coding

In this letter, we propose a vocal tract length (VTL) perturbation method for text-dependent speaker verification (TD-SV), in which a set of TD-SV systems are trained, one for each VTL factor, and score-level fusion is applied to make a final decision. Next, we explore the bottleneck (BN) feature extracted by training deep neural networks with a self-supervised objective, autoregressive predictive coding (APC), for TD-SV and compare it with the well-studied speaker-discriminant BN feature. The proposed VTL method is then applied to APC and speaker-discriminant BN features. In the end, we combine the VTL perturbation systems trained on MFCC and the two BN features in the score domain. Experiments are performed on the RedDots challenge 2016 database of TD-SV using short utterances with Gaussian mixture model-universal background model and i-vector techniques. Results show the proposed methods significantly outperform the baselines.

==> References <==
@inproceedings{michelsanti2017conditional,
  title={{C}onditional Generative Adversarial Networks for Speech Enhancement and Noise-Robust Speaker Verification},
  author={Michelsanti, D. and Tan, Z.-H.},
  booktitle={Proc. of Interspeech},
  pages={2008--2012},
  year={2017},
}

@Article{Mahalanobis36,
	author={P. C. Mahalanobis},
	title={{O}n the {G}eneralised {D}istance in {S}tatistics},
	journal={Proc. of the National Institute of Sciences of India},
        volume={2},
	pages={49-55},
	year={1936}
}


@Article{MacQueen67,
	author={J. MacQueen},
	title={{S}ome {M}ethods for {C}lassification and {A}nalysis of {M}ultivariate {O}bservations},
	journal={Proc. Fifth Berkeley Symp. on Math. Statist. and Prob. (Univ. of Calif. Press)},
	volume={1},
	pages={281-297},
	year={1967}
}

@Article{ross74,
	author={M. J. Ross and  H. L. Shaffer and A. Cohen and R. Freudberg and H. J.Manley},
	title={{A}verage {M}agnitude {D}ifference {F}unction {P}itch {E}xtractor},
	journal={IEEE Trans. Acoust. Speech Signal Processing},
	volume={22},
	pages={353-362},
	year={1974}
}

@INPROCEEDINGS{Makhoul75,
	author = {J. Makhoul},
	title = {{L}inear {P}rediction: {A} {T}utorial {R}eview},
	booktitle = {Proceedings of the IEEE},
	volume={63},
	pages={561-580},
	year={1975}
}

@Article{Sambur76,
	author = {M. R. Sambur},
	title = {{S}peaker {R}ecognition using {O}rthogonal {L}inear {P}rediction},
	journal={IEEE Trans. Acoust. Speech Signal Processing},
	volume={24},
	pages={283-289},
	year={1976}
}
	
@Article{Markel77,
	author = {J. D. Markel and B. T. Oshika and Jr. A. M. Gray},
	title = {{L}ong-term {F}eature {A}veraging for {S}peaker {R}ecognition},
        journal={IEEE Trans. Acoust. Speech Signal Processing},
	volume={25},
	pages={330-337},
	year={1977}
}

@Article{dempster77,
  author={A. Dempster and N. Laird and D. Rubin},
  title={{M}aximum {L}ikelihood from {I}ncomplete {D}ata via {EM} {A}lgorithm},
  journal={J. Roy. statist. Soc.},
  volume={39},
  pages={1-38},
  year={1977}
   }

@Article{Davis80,
	author={S. B. Davis and P. Mermelstein},
	title={{C}omparison of {P}arametric {R}epresentations for {M}onosyllabic {W}ord {R}ecognition in {C}ontinuously {S}poken {S}entences},
	journal={IEEE Trans. Acoust. Speech Signal Processing},
	volume={28},
	pages={357-366},
	year={1980}
}

@Article{LINDE80,
	author={Y. Linde and A. Buzo and  R. M. GRAY},
        title={{A}n {A}lgorithm for {V}ector {Q}uantizer {D}esign},
	journal={IEEE Trans. Communications},
	volume={28},
	pages={84-94},
	year={1980}
}

@Article{Furui81,
	author={S. Furui},
	title={{C}epstral {A}nalysis {T}echnique for {A}utomatic {S}peaker {V}erification},
	journal={IEEE Trans. on  Acoust. Speech Signal Processing},
	volume={29},
	pages={254-272},
	year={1981}
}

@Article{Rabiner89,
	author={L. R. Rabiner},
	title={{A} {T}utorial on {H}idden {M}arkov {M}odels and {S}elected {A}pplications in {S}peech {R}ecognition},
	journal={Proc. of the IEEE},
	volume={77},
	pages={257-285},
	year={1989}
}



@Article{Hermansky90,
	author={H. Hermansky},
	 title={{P}erceptual {L}inear {P}redictive ({PLP}) {A}nalysis of {S}peech},
	 journal={J. Acoust. Soc. Am.},
	 volume={87},
	 pages={1738-1752},
	 year={1990}
}

@Article{Higgin91,
author="A. Higgins and L. Bahler and J. Porter",
title="{S}peaker {V}erification using {R}andomized {P}hrase {P}rompting",
journal="Digital Signal Processing",
volume="1",
 pages="89-106",
year="1991"	 
}

@INPROCEEDINGS{reynolds91,
	author = {D. A. Reynolds and L. P. Heck},
	title = {{I}ntegration of {S}peaker and {S}peech {R}ecognition {S}ystems},
         booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
	 pages = {869-872},
	year = {1991}
}


@INPROCEEDINGS{Rosenberg92,
	author = {A. E. Rosenberg and J. DeLong and C\-H Lee and B\-H Jaung and F. K. Soong},
	title = {{T}he {U}se of {C}ohort {N}ormalized {S}cores for {S}peaker {V}erification},
	booktitle = { Proc. of Int. Conf. Spoken Language Processing (ICSLP)},
	pages = {599-602},
	year = {1992}
}

@Article{Hermanksy94,
       author = {H. Hermanksy and N. Morgan},
       title = {{R}ASTA processing of speech},
       journal={IEEE Trans. on Speech and Audio Processing},
       volume={2},
       pages={578-589},
       year={1994}
}

@Article{Gauvain94,
	author = {J.-L. Gauvain and C.-H. Lee},
	title = {{M}aximum a {P}osteriori {E}stimation for {M}ultivariate {G}aussian {M}ixture {O}bservations of {M}arkov {C}hains},
	journal={IEEE Trans. on Speech and Audio Processing},
	volume={2},
	pages={291-298},
	 year={1994}
}


@Article{reynold95,
  author="D. A. Reynolds",
  title="{S}peaker {I}dentification and {V}erification using {G}aussian {M}ixture {S}peaker {M}odels",
  journal="Speech Communication",
  volume="17",
  pages="91-108",
  year="1995"
}

@Article{Leggeter95,
author="C. Leggetter and P. Woodland",
title="{M}aximum {L}ikelihood {L}inear {R}egression for {S}peaker {A}daptation of {H}MMs",
journal="Computer Speech and Language",
volume="9",
pages="171-186",
year="1995"	
}
@Article{Vapnik95,
	author={C. Cortes and V. Vapnik},
	title={{S}upport {V}ector {N}etworks},
	journal={Machine Learning},
	volume={20},
	pages={273-297},
	year={1995}
}

@INPROCEEDINGS{Talkin95,
	author = {D. Talkin},
        title = {{A} {R}obust {A}lgorithm for {P}itch {T}racking ({RAPT})},
	booktitle = {in Speech coding and synthesis (Elsevier, ed.)},
	pages = {495-518},
        year = {1995}
}

@INPROCEEDINGS{leerose96,
 author = {Li Lee and Richard C. Rose},
 title = {{S}peaker {N}ormalization using {E}fficient {E}requency {W}arping {P}rocedures},
 booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
 pages = {353-356},
 year = {1996}
}



@INPROCEEDINGS{Rosenberg96,
	 author = {A. E. Rosenberg and S. Parthasarathy},
	 title = {{S}peaker {b}ackground {m}odels for {c}onnected {d}igit {p}assword {s}peaker {V}erification},
	 booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
	 pages = {81-84},
	 year = {1996}
}




@INPROCEEDINGS{LHeck97,
	  author = {L. Heck and M. Weintraub},
	  title = {{H}andset-dependent {B}ackground {M}odels for {R}obust {T}ext-{I}ndependent {S}peaker {R}ecognition},
          booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
	  pages = {1071-1074},
	  year = {1997}
}


@INPROCEEDINGS{DET97,
	   author = {A. Martin and G. Doddington and T. Kamm and M. Ordowskiand and M. Przybocki},
	   title = {{T}he {D}ET {C}urve in {A}ssessment of {D}etection {T}ask {P}erformance},
	   booktitle = {Proc. of Eur. Conf. Speech Commun. and Tech. (Eurospeech)},
	   pages = {1895-1898},
	   year = {1997}
}  


@INPROCEEDINGS{Ariyaeeinia97,
	author= {A. M. Ariyaeeinia and P. Sivakumaran},
	title = {{A}nalysis and {C}omparison of {S}core {N}ormalization {M}ethods for {T}ext {D}ependent {S}peaker {V}erification},
	booktitle = {Proc. of Eur. Conf. Speech Commun. and Tech. (Eurospeech)},
        pages = {1379-1382},
	year = {1997}
}


@article{Lee-Rose98,
      author="L. Lee and R. Rose",
      title="{F}requency warping approach  to speaker normalization",
      journal="IEEE Trans. on Speech and Audio Processing",
      volume={6},
      pages={49-59},
      year={1998}
}



@INPROCEEDINGS{reycls98,
	author= {D. A. Reynolds and et. al},
	title = {{B}lind {C}lustering of {S}peech {U}tterances {B}ased on {S}peaker and {L}anguage {C}haracteristics},
	booktitle = {Proc. of Int. Conf. Spoken Language Processing (ICSLP)},
	pages = {3193-3196},
	year={1998}
}

@INPROCEEDINGS{Hermansky98,
	author={S. Van Vuuren and H. Hermansky},
	title={{O}n the {I}mportance of {C}omponents of the {M}odulation {S}pectrum for {S}peaker {V}erification},
        booktitle = {Proc. of Int. Conf. Spoken Language Processing (ICSLP)},
	pages = {3205-3208},
	year = {1998}
}


@Article{Pellom98,
    author={B. L. Pellom and J. H. L. Hansen},
    title={{A}n {E}fficient {S}coring {A}lgorithm for {G}aussian {M}ixture {M}odel {B}ased {S}peaker {I}dentification},
    journal={IEEE Signal Proc. Lett.},
    volume={5},
    pages={281-284},
    year={1998}
}

@Article{HLDA98,
	author= {N. Kumar and A.G. Andreou},
	title={{H}eteroscedastic {D}iscriminant {A}nalysis and {R}educed {R}ank {HMMs} for {I}mproved {S}peech {R}ecognition},
	journal={Speech Communication},
	volume={26},
	pages={283-297},
	year={1998}
}

@INPROCEEDINGS{Isobe99,
	author= {T. Isobe and J. Takahashi},
	title = {{A} {N}ew {C}ohort {N}ormalization using {L}ocal {A}coustic {I}nformation for {S}peaker {V}erification},
	booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
        pages = {841-844},
	year={1999}
}

@INPROCEEDINGS{McLaugn99,
     author={J. McLaughlin and D. A. Reynolds and T. Gleason},
     title={{A} {S}tudy of {C}omputation {S}peed-ups of the {GMM-UBM} {S}peaker {R}ecognition {S}ystem},
     booktitle = {Proc. of Eur. Conf. Speech Commun. and Tech. (Eurospeech)},
     pages={1215-1218},
     year={1999}
}

@INPROCEEDINGS{Markowitz99,
	author={J. Markowitz},
       title={{I}eri and {O}ggi {D}omani: {S}peaker {R}ecognition {Y}esterday, {T}oday and tomorrow},
       booktitle = {Proc. of COST250 Workshop on Speacker Recognition in Telephony},
       year={1999}
}


@INPROCEEDINGS{Auckenthaler1999,
author={R. Auckenthaler and  E. Parris and  M. Carey},
title={{I}mproving a {GMM} {S}peaker {V}erification {S}ystem by {P}honetic {W}eighting},
booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
 pages={313-316},
 year={1999}
}


@Article{kuhn2000,
author="R. Kuhn and J.-C. Junqua and P. Nguyen and N. Niedzielski",
title="{R}apid {S}peaker {A}daptation in {E}igenvoice {S}pace",
journal="IEEE Trans. on Speech and Audio Processing",
volume="8 (6)",
pages="695-707",
year="2000"	
}	  

@Article{reynold00,
  author="D. A. Reynolds and T. F. Quatieri and R. B. Dunn",
  title="{S}peaker verification using adapted Gaussian mixture models",
  journal="Digital Signal Processing",
  volume="10",
  pages="19-41",
 year="2000"	  
}

@Article{Tnorm00,
 author="R. Auckenthaler and M. Carey and H. Lloyd-Thomas",
 title="{S}core {N}ormalization for {T}ext-{I}ndependent {S}peaker {V}erification {S}ystem",
 journal="Digital Signal Processing",
 Volume="10",
 pages="42-54",
 year="2000"
 }


@INPROCEEDINGS{Wagner00,
     author= {D. Tran and M. Wagner},
     title = {{A} {P}roposed {L}ikelihood {T}ransformation for {S}peaker {V}erification},
     booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
     pages = {1069-1072},
     year={2000}
}


@Article{kishore00,
  author="S. P. Kishore and B. Yegnanarayana",
  title="{S}peaker {V}erification: {M}inimizing the {C}hannel {E}ffects using {A}utoassociative {N}eural {N}etwork {M}odels",
  journal="ICASSP",
  year="2000",
  pages="1101-1104"
}



@INPROCEEDINGS{Heck00,
	author= {R. Teunen and B. Shahshahani and L. Heck},
	title = {{A} {M}odel-based {T}ransformational {A}pproach to {R}obust {S}peaker {R}ecognition},
	booktitle = {Proc. of Int. Conf. Spoken Language Processing (ICSLP)},
        pages = {495-498},
        year={2000}
}

@INPROCEEDINGS{paliwal00,
	author= {B. Wildermoth and K. K. Paliwal},
	title = {{U}se of {V}oicing and {P}itch {I}nformation for {S}peaker {R}ecognition},
	booktitle = {Proc. 8th Australian Intern. Conf. Speech Science and Technology},
	pages = {324-328},
       year={2000}

}


@INPROCEEDINGS{Gadde2000,
	author= {V. R. R. Gadde},
	title = {{M}odeling {W}ord {D}uration},
        booktitle = {Proc. of Int. Conf. Spoken Language Processing (ICSLP)},
	pages = {601-604},
        year={2000}
}

@INPROCEEDINGS{Wan2000,
	author= {V. Wan and W. M. Campbell},
	title = {{S}upport {V}ector {M}achines for {S}peaker {V}erification and {I}dentification},
	booktitle = {Proc. IEEE Signal Processing Society Workshop Neural Networks},
	pages = {775-784},
	year={2000}
}


@INPROCEEDINGS{Doddington2001,
        author= {G. Doddington},
        title = {{S}peaker {R}ecognition {B}ased on {I}diolectal {D}ifferences {B}etween {S}peakers},
        booktitle = {Proc. of Eur. Conf. Speech Commun. and Tech. (Eurospeech)},
        pages = {2521-2524},
        year={2001}
}  


@INPROCEEDINGS{Sturim01,
        author= {D. Sturim and D. A. Reynolds and E. Singer and J. P. Campbell},
        title = {{S}peaker {I}ndexing in {L}arge {A}udio {D}atabases using {A}nchor {M}odels},
	booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
	 pages = {429-432},
        year={2001}
}

@INPROCEEDINGS{Auck01,
       author={R. Auckenthaler and J. S. Masion},
       title={{G}aussian {S}election {a}pplied to {T}ext-{I}ndependent {S}peaker {V}erification},
       booktitle = {Proc. of Odyssey Speaker and Language Recognition Workshop},
       pages={83-88},
       year={2001}
}

@INPROCEEDINGS{Pelecanos01,
       author={J. Pelecanos and S. Sridharan},
       title={{F}eature {W}arping for {R}obust {S}peaker {V}erification},
       booktitle = {Proc. of Odyssey Speaker and Language Recognition Workshop},
       pages={213-218},
       year= {2001}
}


@INPROCEEDINGS{Wang2001,
        author= {J. C. N. Wang and W. H. Tsai and L. S. Lee},
        title = {{E}igen-{MLLR} {C}oefficients as {N}ew {F}eature {P}arameters for {S}peaker {I}dentification},
        booktitle = {Proc. of Eur. Conf. Speech Commun. and Tech. (Eurospeech)},
	pages = {1385-1388},
        year={2001}
}


@INPROCEEDINGS{Kajarekar2001,
author= {S. Kajarekar and H. Hermansky},
title = {{S}peaker {V}erification {B}ased on {B}road {P}honetic {C}ategories},
booktitle = {Proc. of Odyssey Speaker and Language Recognition Workshop},
pages={201-206},
year={2001}
}

@INPROCEEDINGS{Glds_ker2002,
	author={W. M. Campbell},
	title={{G}eneralized {L}inear {D}iscriminant {S}equence {K}ernels for {S}peaker {R}ecognition},
	booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
	pages = {161-164},
	year={2002}
}


@INPROCEEDINGS{ReynoldsFmap,
	author= {D.A. Reynolds},
	title = {{C}hannel {R}obust {S}peaker {V}erification via {F}eature {M}apping},
	booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
	pages = {6-10},
        year={2003}
}


@INPROCEEDINGS{Tkinnun03,
    author={T. Kinnunen and E. Karpov and P. Franti},
    title={{A} {S}peaker {P}runing {A}lgorithm for {R}eal-{T}ime {S}peaker {I}dentification},
    booktitle = {Proc. Audio- and Video-Based Biometric Authentication},
    pages={639-646},
        year={2003}
}




@Article{nisteval04,
	author="{T}he {E}valuation {P}lan of NIST 2004 {S}peaker {R}ecognition {C}ampaign.
	http://www.itl.nist.gov/iad/mig//tests/sre/2004/SRE-04\_evalplan{-}v1a.pdf"
}

@INPROCEEDINGS{bonastre04,
        author = {J. F. Bonastre and N. Scheffer and C. Fredouille and D. Matrouf},
        title = {{N}IST'04 {S}peaker {R}ecognition {E}valuation {C}ampaign: {N}ew {LIA} {S}peaker {D}etection {P}lateform based on {ALIZE} {T}oolkit},
        booktitle = {Proc. of NIST 2004 Speaker Recognition Workshop},
        year = {2004},
}

@INPROCEEDINGS{Binma04,
	author = {B. Ma and H. Meng},
	title = {{E}nglish-{C}hinese {b}ilingual {t}ext-independent {s}peaker {v}erification},
	booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
	year={2004}
}

@INPROCEEDINGS{Leung04,
	author = {K. Y. Leung and M. W. Mak and S. Y. Kung},
	title = {{A}pplying {a}rticulatory {f}eatures to {t}elephone-based {s}peaker {v}erification},
        booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
	year={2004}
}

@INPROCEEDINGS{Kwong04,
	author = {Q.Y. Hong and S. Kwong},
	title = {{D}iscriminative {t}raining for {s}peaker {i}dentification based on {m}aximum {m}odel {d}istance {a}lgorithm},
        booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
	year={2004}
}


@ARTICLE {Bimbot04,
author = {F. Bimbot and J.-F. Bonastre and others},
journal = {EURASIP Journal on Applied Signal Processing},
pages = {430-451},
title = {A Tutorial on Text-Independent Speaker Verification},
volume = {4},
year = {2004}
}


@INPROCEEDINGS{Louradour05,
	author = {J. Louradour and K. Daoudi and R. Andre-Obrecht},
	title = {{D}iscriminative {P}ower of {T}ransient {F}rames in {S}peaker {R}ecognition},
	booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
	pages={613-616},
	year={2005}
}



@INPROCEEDINGS{Stolcke05,
	author= {A. Stolcke and L. Ferrer and S. Kajarekar and E. Shriberg and A. Venkataraman},
	title = {{MLLR} {T}ransforms as {F}eatures in {S}peaker {R}ecognition},
        booktitle = {Proc. of Eur. Conf. Speech Commun. and Tech. (Eurospeech)},
	pages = {2425-2428},
        year={2005}
}





@Article{kenny05,
author="P. Kenny",
title="{J}oint {F}actor {A}nalysis of {S}peaker and {S}ession {V}ariability : {T}heory and {A}lgorithms",
journal="Technical report CRIM-06/08-13  Montreal, CRIM",
year="2005"
}



@INPROCEEDINGS{AT_norm,
	author= {D. E. Sturim and D.A. Reynolds},
	title = {{S}peaker {A}daptive {C}ohort {S}election for {T}norm in {T}ext-independent {S}peaker {V}erification},
        booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
	pages = {741-744},
        year={2005}
}	


@INPROCEEDINGS{datadriven05,
	author= {M. Mason and R. Vogt and B. Baker and S. Sridharan},
	title = {{D}ata-{D}riven {C}lustering for {B}lind {F}eature {M}apping in {S}peaker {V}erification},
	booktitle = {Proc. of Interspeech},
         pages = {3109-3112},
        year={2005}
}


@INPROCEEDINGS{ZTnorm05,
	author= {R. Vogt and B. Baker and S. Sridharan},
	title = {{M}odeling {S}ession {V}ariability in {T}ext-{I}ndependent {S}peaker {V}erification},
	booktitle = {Proc. of Eur. Conf. Speech Commun. and Tech. (Eurospeech)},
	pages = {3117-3120},
	year={2005}
}

@INPROCEEDINGS{Adami05,
	author= {André G. Adami},
        title = {{P}rosodic {M}odeling for {S}peaker {R}ecognition based on {S}ub-band {E}nergy {T}emporal {T}rajectories},
	booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
	 pages = {189 - 192},
        year={2005}
}

@INPROCEEDINGS{NAP2005,
	author= {A. Solomonoff and W. M. Campbell and I. Boardman},
	title = {{A}dvances in {C}hannel {C}ompensation for {SVM} {S}peaker {R}ecognition},
	booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
	pages = {629 - 632},
	year={2005}
}
@INPROCEEDINGS{Campbel_GMM_sup06,
author= {W. Campbell and D. Sturim and D. Reynolds and A. Solomonoff},
title = {{SVM} based {S}peaker {V}erification using a {GMM} {S}upervector {K}ernel and {NAP} {V}ariability {C}ompensation},
 booktitle = { Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
 pages = {97-100},
 year={2006}
}

@INPROCEEDINGS{Goldberger05adistance,
author = {J. Goldberger and H. Aronowitz},
title = {{A} {D}istance {M}easure {B}etween {GMM}s {B}ased on the {U}nscented {T}ransform and its {A}pplication to {S}peaker {R}ecognition},
booktitle = {in Proc. of Interspeech},
pages = {1985-1989},
year = {2005}
}



@INPROCEEDINGS{krause06,
	author = {N. Krause and R. Gazit},
	title ={{SVM}-based Speaker {C}lassification in the {GMM} {M}odels {S}pace},
	booktitle = {Proc. of Odyssey Speaker and Language Recognition Workshop},
	year ={2006}
}


@INPROCEEDINGS{Noor06,
	  author = { E. Noor and H. Aronowitz},
	  title={{E}fficient {L}anguage {I}dentification using {A}nchor {M}odels and {S}upport {V}ector {M}achines},    
	  booktitle = {Proc. of Odyssey Speaker and Language Recognition Workshop},
	  year ={2006}
}



@inproceedings{Schwarz,
author = {Schwarz, P. and Matejka, P. and Cernocky, J.},
booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
pages = {325--328},
title = {{H}ierarchical {S}tructures of {N}eural {N}etworks for {P}honeme {R}ecognition},
year = {2006}
}


@INPROCEEDINGS{Binma06,
	author = {B. Ma and D. Zhu and R. Tong and H. Li},
	title={{S}peaker {C}luster {B}ased {GMM} {T}okenization for {S}peaker {R}ecognition},
	booktitle = {Proc. of Interspeech},
        year ={2006},
}


@INPROCEEDINGS{Hazen06,
  author="R. Woo and A. Park and T. J. Hazen",
  title="{T}he {MIT} {M}obile {D}evice {S}peaker {V}erification {C}orpus: {D}ata {C}ollection and {P}reliminary {E}xperiments",
  booktitle="Proc. of Odyssey Speaker and Language Recognition Workshop",
  pages="1-6",
  year="2006"
}


@Article{Campbell2006,
	author={W. M. Campbell and D. E. Sturim and D. A. Reynolds},
	title={{S}upport {V}ector {M}achines using {GMM} {S}upervectors for {S}peaker {V}erification},
	 journal={IEEE Signal Process. Lett.},
	 volume={13},
	 pages={308-311},
	 year={2006}
}


@Article{Mami06,
	author="Y. Mami and D. Charlet",
	title="{S}peaker {R}ecognition by {L}ocation in the {S}pace of {R}eference {S}peakers",
	journal="Speech Communication",
	volume="48",
	pages="127-141",
	year="2006"
}

@Article{Skosan06,
	author={M. Skosan and D. Mashao},
	title={{M}odified {S}egmental {H}istogram {E}qualization for {R}obust {S}peaker {V}erification},
	journal={Pattern Recogn. Lett.},
        volume={27},
        pages={479–486},
        year={2006}
}	


@INPROCEEDINGS{hatch06,
   author = {A. Hatch and S. Kajarekar and A. Stolcke},
   title={{W}ithin-{C}lass {C}ovariance {N}ormalization for {SVM}-{B}ased {S}peaker {R}ecognition},
   booktitle = {Proc. of Int. Conf. Spoken Language Processing (ICSLP)},
   pages = {1471-1474},
   year ={2006}
}


@Article{htkbook,
  author="S. Young and D. Kershaw and J. Odell and V. Valtchev and P. Woodland and et al.",
  title="{HTK} book",
  journal={Copyright 2001-2006 Cambridge University Engineering Department}
   }


@Article{Castro2007,
      author="D. R. Castro and et. al",
      title="{S}peaker {V}erification using {S}peaker- and {T}est-dependent {F}ast {S}core {N}ormalization",
      journal="Pattern Recogn. Lett.",
      volume="28",
      pages="90-98",
      year="2007"
}

@INPROCEEDINGS{Charbuillet07,
	author={C. Charbuillet and B. Gas and M. Chetouani and J. L. Zarader},
	title={{C}omplementary {F}eatures for {S}peaker {V}erification based on {G}enetic {A}lgorithms},
        booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
	pages={285-288},
	year = {2007}
}

@INPROCEEDINGS{Xugang07,
	author={X. Lu and J. Dang},
	 title={{P}hysiological {F}eature {E}xtraction for {T}ext {I}ndependent {S}peaker {I}dentification using {N}on-{U}niform {S}ub-band {P}rocessing},
        booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
	pages={461-464},
        year = {2007}
}

@INPROCEEDINGS{Saeidi07,
	author={R. Saeidi and H. R. Sadegh Mohammadi and R. D. Rodman and T Kinnunen},
	title={{A} {N}ew {S}egmentation {A}lgorithm {C}ombined with {T}ransient {F}rames {P}ower for {T}ext {I}ndependent {S}peaker {V}erification},
	booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
	pages={305-308},
	year = {2007}
}
		
@INPROCEEDINGS{Tur2007,
	author={G. Tur and E. Shriberg and A. Stolcke and S. Kajarekar},
	title={{D}uration and {P}ronunciation {C}onditioned {L}exical {M}odeling for {S}peaker {S}erification},
        booktitle = {Proc. of Interspeech},
	pages={2049-2052},
	year = {2007}
}

@Article{HLDA_feat07,
	author={L. Burget and  P. Matejka and  O. Glembek and P. Schwarz and J. Cernocky},
        title = {{A}nalysis of {F}eature {E}xtraction and {C}hannel {C}ompensation in {GMM} {S}peaker {R}ecognition {S}ystem},
	journal={IEEE Trans. on Audio, Speech, Lang. Process.},
	volume={15},
	pages={1979-1986},
	year={2007}
}

@Article{fusion_2007,
	 author={N. Brummer and L. Burget and J. Cernocky and others},
	 title = {{F}usion of {H}eterogeneou {S}peaker {R}ecognition {S}ystems in the {STBU} {S}ubmission for the {NIST} {S}peaker {R}ecognition {E}valuation 2006},
	 journal={IEEE Trans. on Audio, Speech, and Lang. Process.},
	 volume={15},
	 pages={2072-2084},
	 year={2007}
}

@INPROCEEDINGS{Hazen97,
       author= {T. J. Hazen and J. R. Glass},
       title = {{A} {C}omparison of {N}ovel {T}echniques for {I}nstantaneous {S}peaker {A}daptation},
       booktitle = {Proc. of Eur. Conf. Speech Commun. and Tech. (Eurospeech)},
       pages = {2047-2050},
       year = {1997}
}


@INPROCEEDINGS{ferras-icassp08,
	author = {M. Ferras and  C. C. Leung and C. Barras and J. L. Gauvain},
        title = {{C}onstrained {MLLR} for {S}peaker {R}ecognition},
	booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
	pages = {53-56},
	year = {2007}
}


	       


@inproceedings{akhil-interspeech2008,
      author = {P. T. Akhil and S. P. Rath and S. Umesh and D. R. Sanand},
      title = {{A} computationally efficient approach to warp factor estimation in VTLN using EM algorithm and sufficient satistics},
      booktitle = {Proc. of Interspeech},
      pages = {1713-1716},
      year = {2008}
}


@inproceedings{sanand-interspeech2008,
      author={D. R. Sanand and S. Umesh},
      title={{S}tudy of {J}acobian {C}ompensation Using {L}inear {T}ransformation of {C}onventional {MFCC} for {VTLN}},
      booktitle={Proc. of Interspeech},
      pages={1233-1236},
      year={2008}
}




@inproceedings{Yossi09,
	author = {Y. Bar-Yosef and Y. Bistritz},
        title = {{A}daptive {I}ndividual {B}ackground {M}odel for {S}peaker {V}erification},
        booktitle = {Proc. of Interspeech},
	pages = {1271-1274},
	year = {2009}
}	

@Article{Vraj09,
	author="V. R. Apsingekar and P. L. De Leon",
	title="{S}peaker {M}odel {C}lustering for {E}fficient {S}peaker {I}dentification in {L}arge {P}opulation {A}pplications",
	journal="IEEE Trans. on Speech and Language Processing",
	volume="17",
	pages="848-853",
	year="2009"
}


@article{kinnunen2010overview,
  title={{A}n overview of text-independent speaker recognition: from features to supervectors},
  author={Kinnunen, T. and Li, H.},
  journal={Speech communication},
  volume={52},
  number={1},
  pages={12--40},
  year={2010}
 }



@inproceedings{achintya-odyssey2010,
	author= {A. K. Sarkar and S. Umesh},
	title= {{I}nvestigation of Speaker-Clustered UBMs based on Vocal Tract Lengths and MLLR matrices for Speaker Verification},
	booktitle={Proc. of Odyssey Speaker and Language Recognition Workshop},
	pages= {286-293},
	year = {2010}

}

@inproceedings{achintya-odyssey2010_spkid,
	      author= {A. K. Sarkar and S. Umesh and S. P. Rath},
	      title= {{C}omputationally {E}fficient {S}peaker {I}dentification for {L}arge {P}opulation {T}asks using {MLLR} and {S}ufficient {S}tatistics},
	      booktitle={Proc. of Odyssey Speaker and Language Recognition Workshop},
	      pages= {7-11},
              year = {2010}
}


@inproceedings{Zhang-odyssey2010,
       author= {W. Q. Zhang and Y. Shan and J. Liu},
       title= {{M}ultiple Background Models for Speaker Verification},
       booktitle={Proc. of Odyssey Speaker and Language Recognition Workshop},
       pages={47-51},
       year = {2010}
}



@inproceedings{achintya-inter2010,
             author= {A. K. Sarkar and S. Umesh},
             title= {{F}ast {C}omputation of {S}peaker {C}haracterization {V}ector using {MLLR} and {S}ufficient {S}tatistics in {A}nchor {M}odel {F}ramework},
             booktitle = {Proc. of Interspeech},
	     pages={2738-2741},
	     year = {2010}
}


@inproceedings{achintya-icassp2011,
	        author= {A. K. Sarkar and S. Umesh},
	        title= {{U}se of VTL-wise Models in Feature-Mapping Framework to Achieve Performance of Multiple-Background Models in Speaker Verification},
	        booktitle={Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
		pages={4552-4555},
	        year = {2011}

}

@inproceedings{SenoussaouiInterspch2011,
        author= {M. Senoussaoui and others},
        title= {{M}ixture of plda models in I-vector space for gender-independent speaker recognition},
        booktitle={Proc. of Interspeech},
        pages={25-28},
         year = {2011}
}


@Article{Deka_ieee2011,
       author= {N. Dehak and P. Kenny and R. Dehak and P. Ouellet and P. Dumouchel},
       title= {{F}ront-end factor analysis for speaker verification},
       journal={IEEE Trans. on Audio, Speech and Language Processing},
       volume={19},
       pages={788-798},
       year = {2011}
}

@inproceedings{Romero2011,
        author= {D. G. Romero and C. Y. Espy-Wilson},
        title= {{A}nalysis of i-vector {L}ength {N}ormalization in {S}peaker {R}ecognition {S}ystems},
        booktitle={Proc. of Interspeech},
        pages={249-252},
        year={2011}
}



@inproceedings{Kanagasundaram2011,
author={A. Kanagasundaram and R. Vogt and D. Dean and  S. Sridharan and M. Mason},
title= {i-vector based {S}peaker {R}ecognition on {S}hort {U}tterances},
booktitle={Proc. of Interspeech},
pages={2341-2344},
year={2011}
}

@inproceedings{Pierre-interspeech2012,
       author= {P. M. Bousquet and others},
       title= {{V}ariance-spectra based normalization for i-vector standard and probabilistic linear discriminant anal
ysis},
       booktitle={Proc. of  Odyssey Speaker and Language Recognition Workshop},
       year={2012},
       pages = {157-164}
}

@inproceedings{Larcher2012,
author= {A. Larcher and K. A. Lee and  B. Ma and H. Li},
title= {{RSR2015}: database for text-dependent speaker verification using multiple pass-phrases},
booktitle={Proc. of Interspeech},
pages={1580-1583},
 year = {2012}
}

@inproceedings{achintya2012,
author={A. K. Sarkar and  D. Matrouf and P. M. Bousquet and J. F. Bonastre},
title= {{S}tudy of the Effect of i-vector Modeling on Short and Mismatch Utterance Duration for Speaker Verification},
booktitle={Proc. of Interspeech},
pages={2662-2665},
year={2012}
}




@inproceedings{Plchot2013,
author={O. Plchot and others},
title={{D}eveloping  a  {S}peaker  {I}dentification {S}ystem  for the {DARPA} {RATS} {P}roject},
booktitle={Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
pages={ 6768-6772},
year={2013}
}





@inproceedings{Fu2014,
author={T. Fu and Y. Qian and Y. Liu and Kai Yu}, 
title= {{T}andem deep features for text-dependent speaker verification},
booktitle={Proc. of Interspeech},
pages={1327-1331},
year = {2014}
}

@inproceedings{Nicolas2014,
author={N. Scheffer and Y. Lei},
title= {{C}ontent {M}atching for {S}hort {D}uration {S}peaker {R}ecognition},
booktitle={Proc. of Interspeech},
pages={1317-1321},
year = {2014}
}

@inproceedings{Hagai2014,
author={H. Aronowitz and  A. Rendel},
title= {{D}omain {A}daptation for {T}ext {D}ependent {S}peaker {V}erification},
booktitle={Proc. of Interspeech},
pages={1337-1341},
year = {2014}
}


@Article{RSR2015,
author={A. Larcher and  K. A. Lee and  B. Ma and H. Li},
title= {{T}ext-dependent speaker verification: classifiers, databases and RSR2015},
journal={Speech Communucation},
volume={60},
pages={56-77},
year={2014}
}


@inproceedings{McLaren2015,
author={M. McLaren and Y. Lei and L. Ferrer},
title={{A}dvances in deep neural network approaches to speaker recognition},
booktitle={Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
year={2015},
pages={4814-4818}

}


@Article{Yuan2015,
author={Y. Liu and Y. Qian and N. Chen and T. Fu and Y. Zhang and K. Yu},
title= {{D}eep feature for text-dependent speaker verification},
journal={Speech Communication},
volume={73},
pages={1-13},
year={2015}
}

@inproceedings{Delgado2016Asru,
author={H. Delgado and  M. Todisco and  M. Sahidullah and  A. K. Sarkar and N. Evans and  T. Kinnunen and  Z.-H. Tan},
title={{F}URTHER OPTIMISATIONS OF CONSTANT Q CEPSTRAL PROCESSING FOR INTEGRATED UTTERANCE AND TEXT-DEPENDENT SPEAKER VERIFICATION},
booktitle={Proc. of IEEE Spoken Language Technology Workshop (SLT)},
year={2016}
}

@misc{CNTK,
author= {A. Agarwal and others},
title= {{A}n {I}ntroduction to {C}omputational {N}etworks and the {C}omputational {N}etwork {T}oolkit},
year={2016},
howpublished ={https://www.microsoft.com/en-us/research/publication/an-introduction-to-computational-networks-and-the-computational-network-toolkit/}
}

@article{Tang2016,
author = {H. Tang},
title= {{S}equence {P}rediction with {N}eural {S}egmental {M}odels},
journal = {Ph.D. dissertation, Dept. Comput. Sci., Toyota Technological Inst. Chicago,
Chicago, IL, USA},
year =  {2017}
}


@inproceedings{yu2017adversarial,
  title={{A}dversarial Network Bottleneck Features For Noise Robust Speaker Verification},
  author={Yu, H. and Tan, Z.-H. and Ma, Z. and Guo, J.},
  booktitle={Proc. of Interspeech},
  pages={1492--1496},
  year={2017}
}



@article{tang2017endtoend,
  title = {{E}nd-to-End {N}eural {S}egmental {M}odels {F}or {S}peech {R}ecognition},
  author = {H. Tang and L. Lu and K. Gimpel and K. Livescu and C. Dyer and N. A. Smith and S. Renals},
  year = {2017},
  pages={1254-1264},
  journal = {IEEE Journal of Selected Topics in Signal Processing},
  volume = {11}
}



@article{DBLP:journals/taslp/SarkarTTSG19,
  author    = {A. K. Sarkar and
               Z.-H. Tan and
               H. Tang and
               S. Shon and
               J. R. Glass},
  title     = {{T}ime-Contrastive Learning Based Deep Bottleneck Features for Text-Dependent Speaker Verification},
  journal   = {{IEEE/ACM} Trans. Audio, Speech {\&} Language Processing},
  volume    = {27},
  number    = {8},
  pages     = {1267--1279},
  year      = {2019}
}

@misc{xvector_recipe,
 title= {https://github.com/kaldi-asr/kaldi/tree/master/egs/sre16/v2}
 }
 
@inproceedings{conf/icassp/SnyderGSPK18,
  author    = {D. Snyder and
               D. Garcia{-}Romero and
               G. Sell and
               D. Povey and
               S. Khudanpur},
  title     = {{X}-Vectors: robust DNN Embeddings for Speaker Recognition},
  booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
  pages     = {5329--5333},
   year      = {2018}
}


@Article{alizetoolkit,
  title="http://lia.univ-avignon.fr/heberges/ALIZE/"
   }

@Article{mit_database,
  title="http://groups.csail.mit.edu/sls/mdsvc"
}

@Book{duda_hart_patt,
	  author = {R.O. Duda and P.E. Hart and D.G. Stork},
	  title  = {{P}attern {C}lassification},
	  publisher = {New York: John Wiley \& Sons},
	  year    = {2001}
}


@inproceedings{Timit,
author = {J. S. Garofolo and L. F. Lamel and W. M. Fisher and J. G. Fiscus and  D. S. Pallett and N. L. Dahlgren and V. Zue},
title = {{TIMIT} Acoustic-Phonetic Continuous Speech Corpus LDC93S1},
publisher = {Web Download. Philadelphia: Linguistic Data Consortium},
year={1993}
}


@inproceedings{noise_mix,
author= {A. Hannun and C. Case and J. Casper and B. Catanzaro and G. Diamos and E. Elsen and R. Prenger and S. Satheesh and S. Sengupta and A. Coates and A. Ng},
title = {{D}eep speech: scaling Up End-to-End Speech recognition},
 booktitle= {in arXiv, 2014}
}


@article{Sarkar2017,
author = {A. K. Sarkar and Z.-H. Tan},
title ={{I}ncorporating {P}ass-phrase {D}ependent {B}ackground {M}odels for {T}ext-dependent {S}peaker {V}erification},
journal={ Computer speech \& Language},
volume={47},
year ={2018},
pages= {259-271}
}



@article{journals/taslp/SarkarTTSG19,
  author    = {A. K. Sarkar and Z. -H. Tan and H. Tang and S. Shon and  J. R. Glass},
  title     = {Time-Contrastive {L}earning {B}ased {D}eep {B}ottleneck {F}eatures for {T}ext-Dependent {S}peaker {V}erification},
  journal   = {{IEEE/ACM} Trans. Audio, Speech {\&} Language Processing},
  volume    = {27},
  number    = {8},
  pages     = {1267--1279},
  year      = {2019}
}


@article{Park_2019,
   title={{S}pecAugment: a simple data augmentation method for automatic speech recognition},
    pages={2613--2617},
   author={Park, Daniel S. and Chan, William and Zhang, Yu and Chiu, Chung-Cheng and Zoph, Barret and Cubuk, Ekin D. and Le, Quoc V.},
   year={2019},
   booktitle={Proc. of Interspeech}
}

@INPROCEEDINGS{Jaitly_vocaltract,
    author = {N. Jaitly and G. E. Hinton},
    title = {{V}ocal Tract Length Perturbation VTLP Improves Speech Recognition},
    booktitle = {Proc. of International Conference on Machine Learning (ICML)},
    year = {2013}
}

@INPROCEEDINGS{Mauch2013,
author = {M. Mauch and S. Ewert},
title = {{T}he Audio Degradation Toolbox and its Application to Robustness Evaluation},
year = {2013},
booktitle = {International Society for Music Information Retrieval Conference, ISMIR},
pages = {83-88}
}

@INPROCEEDINGS{Lasseck2018,
author = {M. Lasseck},
title= {{A}udio-based Bird Species Identification with Deep Convolutional Neural Networks},
booktitle = {In: Working Notes of CLEF 2018 (C{r}oss Lan{g}uage Evalu{ation Fo{r}um)}}
}

@misc{Focal,
	author= {N. Brummer},
	title= {{F}oCal {T}oolkit},
	howpublished ={Available at http://sites.google.com/site/nikobrummer/focal}
}

@misc{Lnknet,
title= {http://www.ll.mit.edu/mission/communications/ist/lnknet/index.html}
}
@misc{RedDots,
title= {The RedDots Challenge: Towards Characterizing Speakers from Short Utterances},
howpublished ={https://sites.google.com/site/thereddotsproject/reddots-challenge}
}

@misc{SRE08,
title = {https://www.nist.gov/itl/iad/mig/2008-nist-speaker-recognition-evaluation-results}
}

@ARTICLE{7829341,
author={J. {Salamon} and J. P. {Bello}},
journal={IEEE Signal Processing Letters},
title={{D}eep Convolutional Neural Networks and Data Augmentation for Environmental Sound Classification},
year={2017},
volume={24}, 
number={3},
pages={279-283}
}


@ARTICLE{24792,  
author={F. L. {Bookstein}}, 
journal={IEEE Transactions on Pattern Analysis and Machine Intelligence},  
title={{P}rincipal Warps: thin-plate Splines and the Decomposition of Deformations},
year={1989}, 
volume={11},
number={6}, 
pages={567-585}
}

@ARTICLE{Shorten2019,
author = {C. Shorten and T. M. Khoshgoftaar},
title = {{A} Survey on Image Data Augmentation for Deep Learning},
journal = {Journal of Big Data},
year ={2019}
}


@INPROCEEDINGS{ITU2005,
author = {ITU},
title = {{G.} 191: {S}oftware {T}ools for {S}peech and {A}udio {C}oding {S}tandardization},
booketitle ={International Telecommunication Union},
year = {2005}

}



@INPROCEEDINGS{7528399,  
author={H. {Yu} and A. {Sarkar} and D. A. L. {Thomsen} and Z.-H. {Tan} and Z. {Ma} and J. {Guo}},
booktitle={First International Workshop on Sensing, Processing and Learning for Intelligent Machines (SPLINE)},  
title={{E}ffect of Multi-condition Training and Speech Enhancement Methods on Spoofing Detection},
year={2016}, 
pages={1-5}
}

@INPROCEEDINGS{I4U2013,
author = {R. Saeidi and others},
title = {{I4U} submission to NIST SRE 2012: a large-scale collaborative effort for noise-robust speaker verification},
pages= {1986-1990},
year ={2013},
Booktitle = {Proc. of Interspeech}
}

@INPROCEEDINGS{Stewart2010,
author = {R. Stewart and M. Sandler},
title = {{D}atabase of Omnidirectional and b-format Room Impulse Responses},
booktitle = {Proc. IEEE Intl. Conf. on Acoustics Speech and Signal Processing (ICASSP)},
pages = {165-168},
year={2010}
}

@inproceedings{Hinton2012,
author = {G. Hinton and others},
title = {{D}eep {N}eural {N}etworks {F}or {A}coustic {M}odeling {I}n {S}peech {R}ecognition},
booktitle={IEEE Signal Process. Mag.},
pages={82-97},
year={2012}
}

@INPROCEEDINGS{9053481,
  author={S. {Wang} and J. {Rohdin} and O. {Plchot} and L. {Burget} and K. {Yu} and J. {Černocký}},

  booktitle={ Proc. IEEE Intl. Conf. on Acoustics Speech and Signal Processing (ICASSP)}, 

  title={Investigation of Specaugment for Deep Speaker Embedding Learning}, 
  year={2020},
  pages={7139-7143}
  }
  
  @misc{tensorflow2015-whitepaper,
title={ {TensorFlow}: large-scale machine learning on heterogeneous systems},
url={https://www.tensorflow.org/},
note={Software available from tensorflow.org},
author={M. Abadi and
     others},
  year={2015}
}

@article{TanSD20,
  author    = {Z.-H. Tan and  A. K. Sarkar and N. Dehak},
  title     = {{rVAD}: an unsupervised segment-based robust voice activity detection method},
  journal   = {Computer Speech \& Language},
  volume    = {59},
  pages     = {1--21},
  year      = {2020}
 } 
 
 @INPROCEEDINGS{sarkar2009,
 author = {Sarkar, A. K. and Umesh, S. and Rath, S. P.},
 title={{T}ext-independent speaker identification using vocal tract length normalization for building universal background model},
 booktitle={Prof. of Interspeech},
 year = {2009},
 pages ={2331-2334}
 }
 
 @INPROCEEDINGS{1660171,
  author={B. {Lee} and S. {Yoon} and H. {Kang} and D. H. {Youn}},
  booktitle={Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)}, 
  title={{O}n the Use of Voting Methods for Speaker Identification Based on Various Resolution Filter banks}, 
  year={2006},
  pages={I-I}
  }

@article{DBLP:journals/spl/SarkarDLB14,
  author    = {A. K. Sarkar and C. T. Do and V. B. Le and
               C. Barras},
  title     = {{C}ombination Of Cepstral And Phonetically Discriminative Features For Speaker Verification},
  journal   = {{IEEE} Signal Process. Lett.},
  volume    = {21},
  number    = {9},
  pages     = {1040--1044},
  year      = {2014},
  }
  
  @INPROCEEDINGS{Ragni2014,
  author ={Ragni, Anton and Knill, Kate M. and Rath, Shakti P. and Gales, Mark J. F.},
  title = {{D}ata augmentation for low resource languages},
  booktitle ={Proc. of  INTERSPEECH},
  yaer ={2014},
  pages = {810-814}
  }
  
  
  @INPROCEEDINGS{vtlnubm, 
   author = {Sarkar, A. K. and Umesh, S. and Rath, S. P.},
   title ={{T}ext-independent speaker identification using vocal tract length normalization for building universal background model},
   booktitle ={Proc. of  INTERSPEECH},
   pages = {2331-2334},
   year = {2009}
   }

@inproceedings{chung2020generative,
  title = {{G}enerative pre-training for speech with auto-regressive predictive coding},
  author = {Chung, Y.-A. and Glass, J.},
  booktitle = {Proc of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
  year = {2020},
  pages={3497-3501}
}

@INPROCEEDINGS{7078563,
  author={R. Serizel and D. Giuliani},
  booktitle={IEEE Spoken Language Technology Workshop (SLT)}, 
  title={{V}ocal tract length normalisation approaches to DNN-based children's and adults' speech recognition}, 
  year={2014},
  pages={135-140}
}

@article{umesh_sadana,
author={S. Umesh},
title={{S}tudies on inter-speaker variability in speech
and its application in automatic speech recognition},
journal={Sadhana},
volume={36},
pages= {853-883},
year={2011}
}


@inproceedings{Chung2019,
  author={Y. Chung and W.-N. Hsu and H. Tang and J. Glass},
  title={{A}n Unsupervised Autoregressive Model for Speech Representation Learning},
  year=2019,
  booktitle={Proc. Interspeech},
  pages={146--150},
  }
  
  
@article{zeinali2019short,
  title={Short-duration Speaker Verification (SdSV) Challenge 2020: the Challenge Evaluation Plan},
  author={Zeinali, Hossein and Lee, Kong Aik and Alam, Jahangir and Burget, Lukas},
  journal={arXiv preprint arXiv:1912.06311},
  year={2019}
}

@INPROCEEDINGS{UIAI20,
  author = {M. Sahidullah and A. K. Sarkar and V. Vestman and X. Liu and R. Serizel and T. Kinnunen and  Z.-H. Tan and  E. Vincent},
  title ={{UIAI} System for Short-Duration Speaker Verification Challenge 2020},
  booktitle ={Accepted at Spoken Language Technology (SLT) Workshop},
  year={2021}
  }
  
  @inproceedings{DBLP:conf/icassp/SnyderGSPK18,
  author    = {D. Snyder and
               D. Garcia{-}Romero and
               G. Sell and
               D. Povey and
               S. Khudanpur},
  title     = {{X}-vectors: robust DNN embeddings for speaker recognition},
  booktitle = {Proc. of IEEE Int. Conf. Acoust. Speech Signal Processing (ICASSP)},
  pages     = {5329--5333},
    year      = {2018}
}

